When Does the Gittins Policy Have Asymptotically Optimal Response Time Tail?

We consider scheduling in the M/G/1 queue with unknown job sizes. It is known that the Gittins policy minimizes mean response time in this setting. However, the behavior of the tail of response time under Gittins is poorly understood, even in the large-response-time limit. Characterizing Gittins's asymptotic tail behavior is important because if Gittins has optimal tail asymptotics, then it simultaneously provides optimal mean response time and good tail performance. In this work, we give the first comprehensive account of Gittins's asymptotic tail behavior. For heavy-tailed job sizes, we find that Gittins always has asymptotically optimal tail. The story for light-tailed job sizes is less clear-cut: Gittins's tail can be optimal, pessimal, or in between. To remedy this, we show that a modification of Gittins avoids pessimal tail behavior while achieving near-optimal mean response time.

==> figures/macros.tex <==
\makeatletter

% The calc library needs this.
\catcode`\$=3 % math shift

\usetikzlibrary{backgrounds, math, shapes, positioning, decorations, decorations.pathreplacing}

\def\@above{above}
\def\@below{below}
\def\@left{left}
\def\@right{right}
\def\@negativeud{-}
\def\@negativelr{-}
\newcommand{\flipudmode}{%
  \def\@above{below}
  \def\@below{above}
  \def\@negativeud{}}
\newcommand{\fliplrmode}{%
  \def\@left{right}
  \def\@right{left}
  \def\@negativelr{}}

\newcommand{\xscale}{10}
\newcommand{\yscale}{5}
\newcommand{\ticksize}{4}
\newcommand{\arrowsize}{10}
\newcommand{\xarrowsize}{(\arrowsize/\xscale)}
\newcommand{\yarrowsize}{(\arrowsize/\yscale)}

\newcommand{\xscaleload}{%
  \renewcommand{\xscale}{150}
  \renewcommand{\yscale}{10}}

\newcommand{\projx}[1]{($ (0,0)!#1!(1,0) $)}
\newcommand{\projxheight}[2]{($ (0,#2)!#1!(1,#2) $)}
\newcommand{\midpt}[2]{($ #1!0.5!#2 $)}

\newcommand{\xguide}[3][]{%
  \draw[axis] ({#2}, 0) -- ({#2}, {\@negativeud(\ticksize)/\yscale})
  node[\@below] {\ifempty{#1}{$#2$}{#1}\vphantom{by}};
  \draw[guide] ({#2}, 0) -- ({#2}, {#3});}
\newcommand{\yguide}[3][]{%
  \draw[axis] (0, {#3}) -- ({\@negativelr(\ticksize)/\xscale}, {#3})
  node[\@left] {\ifempty{#1}{$#3$}{#1}};
  \draw[guide] (0, {#3}) -- ({#2}, {#3});}
\newcommand{\yguidenolabel}[2]{%
  \draw[guide] (0, {#2}) -- ({#1}, {#2});}
\newcommand{\xguidept}[2]{%
  \ifempty{#1}{}{
    \draw[axis] \projx{#2} -- \projxheight{#2} {\@negativeud(\ticksize)/\yscale};
  }{
    node[\@below] {#1\vphantom{by}};
  }
  \draw[guide] \projx{#2} -- #2;}

\newcommand{\axes}[6]{%
  \draw[axis, ->] (\@negativelr\ticksize/\xscale, 0)
  node[\@left] {#3$\vphantom{by}$} -- ({\@negativelr(-1)*(#1 + \xarrowsize)}, 0)
  node[\@right] {#4$\vphantom{by}$};
  \draw[axis, ->] (0, \@negativeud\ticksize/\yscale)
  node[\@below] {#5$\vphantom{by}$} -- (0, {#2 + \yarrowsize})
  node[\@above] {#6$\vphantom{by}$};}

\newcommand{\axesxtorsor}[4]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0)
  node[left] {$0$} -- ({#1 + \xarrowsize}, 0) node[right] {#3};
  \draw[axis, ->] (0, 0) -- (0, {#2 + \yarrowsize})
  node[\@above] {#4};}

\newcommand{\point}[2][primary]{%
  \filldraw[#1, thick] #2 circle (1.8mu);}

\newcommand{\jump}[4][primary]{%
  \point[#1, fill=white]{(#2, #3)}
  \point[#1]{(#2, #4)}}

\newcommand{\plotlegend}[1][%
  $\Delta \to 0$ limit \\ (lower bound)]{%
  \node[anchor=west, align=left] at (1.13, 32) {%
    $\Delta = 0$ \\ (exact analysis)};
  \draw[primary] (1.1, 25) -- +(0, 14);
  \node[anchor=west, align=left] at (1.13, 62) {#1};
  \draw[bubble] (1.1, 55) -- +(0, 14);}

\newcommand{\snakefirst}[2]{#1 parabola bend #1 \midpt{#1}{#2}}
\newcommand{\snakesecond}[2]{\midpt{#1}{#2} parabola bend #2 #2}
\newcommand{\snake}[2]{\snakefirst{#1}{#2} -- \snakesecond{#1}{#2}}

\newcommand{\intervallabel}[3]{%
  \begin{scope}
    \node (A) at \projx{#1} {};
    \node (B) at \projx{#2} {};
    \node[\@above=0.5em, inner sep=0pt] at \midpt{(A)}{(B)} {%
      \footnotesize #3\vphantom{ly}};
  \end{scope}}
\newcommand{\intervalsnake}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- \snake{#3}{#4} -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 \snake{#3}{#4};
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalsnakefirst}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- #3 parabola bend #3 #4 -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3 parabola bend #3 #4;
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalsnakesecond}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- #3 parabola bend #4 #4 -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3 parabola bend #4 #4;
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalspecial}[6][--]{%
  \begin{scope}[on background layer]
    \fill[#2]
      \projx{#3}
      -- #3
      parabola bend #4 #4
      parabola bend #4 #5
      -- \projx{#5};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3;
  \intervallabel{#3}{#5}{#6}}
\newcommand{\discarded}[2]{%
  \interval{discarded}{#1}{#2}{}}
\newcommand{\original}[2]{%
  \interval{original}{#1}{#2}{$0$-old}}
\newcommand{\recycled}[3][]{%
  \interval{recycled}{#2}{#3}{\ifempty{#1}{}{$#1$-}old}}

\tikzset{%
  figure/.style={x=\xscale, y=\yscale, thick, font=\small,
    baseline={([yshift={-\ht\strutbox}]current bounding box.north)}},
  axis/.style={semithick},
  guide/.style={black!60, semithick, dotted},
  primary/.style={ultra thick, color=cyan!80!black},
  secondary/.style={ultra thick, color=purple!85!white},
  tertiary/.style={ultra thick, color=green!12!yellow!70!black},
  hill/.style={color=red!33!yellow!25},
  valley/.style={color=green!75!yellow!20}}

\catcode`\$=13 % active
\makeatother

